Formalizing Box Inference for Capture Calculus

Capture calculus has recently been proposed as a solution to effect checking, achieved by tracking the captured references of terms in the types. Boxes, along with the box and unbox operations, are a crucial construct in capture calculus, which maintains the hygiene of types and improves the expressiveness of polymorphism over capturing types. Despite their usefulness in the formalism, boxes would soon become a heavy notational burden for users when the program grows. It thus necessitates the inference of boxes when integrating capture checking into a mainstream programming language. In this paper, we develop a formalisation of box inference for capture calculus. We begin by introducing a semi-algorithmic variant of the capture calculus, from which we derive an inference system where typed transformations are applied to complete missing box operations in programs. Then, we propose a type-level system that performs provably equivalent inference on the type level, without actually transforming the program. In the metatheory, we establish the relationships between these systems and capture calculus, thereby proving both the soundness and the completeness of box inference.

==> figures/adpt-sub.tex <==
\begin{wide-rules}

% \textbf{Type Level Box Adaptation \quad $\adpTypDft{x}{T}{U}$}

% \infrule[Adapt]
% {\typPrecDft{x}{T_0} \\
%   \adpDft{x}{T_0}{t}{T} \\
%   \wfTyp{\G}{T}
% }
% {\adpTypDft{x}{t}{T}}

\textbf{Type Level Box Adaptation \quad $\adptTypDft{x}{U}{\cCat}{C}$}

  \infrule[AdaptT]
  {\typPrecDft{x}{U} \\
  \adptDft{U}{T}{\cCat}{{C_e}} \andalso \wfTyp{\G}{T} \\
  C = \begin{cases}
    C_e \cup \set{x}, &\text{if $\cCat \in \set{\cVar, \cVal, \cTrm}$} \\
    C_e, &\text{otherwise}
  \end{cases}
  }
  {\adptTypDft{x}{T}{\cCat}{C}}

  % \infrule[Box]
  % {\typPrecDft{x}{U_0} \\
  % \adptDft{U_0}{U}{\cCat}{C_e} \andalso \wfTyp{\G}{U} \\
  % % \cCat \in \set{\cVar, \cVal} \\
  % T = C_1\,\tBox{C_2\tBox{\cdots C_n\,\tBox{U}}} \\
  % C_1 \cup \cdots \cup C_n \subseteq \dom{\G} \\
  % C = \begin{cases}
  %   \emptyset, &\text{if $\cCat \in \set{\cVar, \cVal}$} \\
  %   C_e \cup \set{x}, &\text{otherwise}
  % \end{cases}
  % }
  % {\adptTypDft{x}{T}{C}}

  % \infrule[Normal]
  % {\typPrecDft{x}{U_0} \\
  % \adptDft{U_0}{U}{\cCat}{C_e} \andalso \wfTyp{\G}{U}
  % % U \text{ is not in the form of } C_1\,\tBox{C_2\tBox{\cdots C_n\,\tBox{T}}} \\
  % }
  % {\adptTypDft{x}{U}{C_e \cup \set{x}}}

\textbf{Type-Level Adaptation subtyping \quad $\adptDft{T}{U}{\cCat}{C}$}

\begin{multicols}{2}

\infrule[Refl]
  {\subDft{C}{C^\prime}}
  {\adptDft{\tCap{C}{S}}{\tCap{C^\prime}{S}}{\cVar}{\eset}}

\infrule[TVar]
  {X <: S \in \G \\
  \adptDft{\tCap{C}{S}}{\tCap{C^\prime}{S^\prime}}{\cCat}{C}}
  {\adptDft{\tCap{C}{X}}{\tCap{C^\prime}{S^\prime}}{\cCat}{C}}

\infrule[Top]
  {\subDft{C}{C^\prime}}
  {\adptDft{\tCap{C}{S}}{\tCap{C^\prime}{\top}}{\cVar}{\eset}}

\infrule[Boxed]
  {\adptDft{\tCap{C_1}{S_1}}{\tCap{C_2}{S_2}}{\cCat}{C_e}\\
   (\cCat^\prime, C_e^\prime) =
   \begin{cases}
     (\cVar, C_e), &\text{if $\cCat$ is $\cVar$} \\
     (\cTrm, C_1), &\text{if $\cCat$ is $\cVal$} \\
     (\cTrm, C_e \cup C_1), &\text{otherwise} \\
   \end{cases}
   }
  {\adptDft{C_x\,\tBox{\tCap{C_1}{S_1}}}{\tCap{C_y}{\tBox{\tCap{C_2}{S_2}}}}{\cCat^\prime}{C_e^\prime}}

% \infrule[Boxed$_{\textrm{id}}$]
% {\adpTyp{\extendG{y}{\tCap{C}{S_1}}}{y}{y}{\tCap{C'}{S_2}}}
% {\adpDft{x}{\tBox{\tCap{C}{S_1}}}{x}{\tCap{C^{\prime\prime}}{\tBox{\tCap{C^\prime}{S_2}}}}}

% \infrule[Boxed$_{<:}$]
% {\subDft{C}{C^\prime} \\
%   \subDft{\tBox{T_1}}{\tBox{T_2}}}
% {\adptDft{\tCap{C}{\tBox{T_1}}}{\tCap{C^{\prime}}{\tBox{T_2}}}{\eset}}

% \infrule[Fun$_{\textrm{id}}$]
% {\adpTyp{\extendG{x}{U_2}}{x}{x}{U_1} \\
%   \adpTyp{(\G, x: U_1, z: T_1)}{z}{z}{T_2}\\
%   \subDft{C}{C^\prime}
% }
% {\adpDft{x_f}{C\,\tForall{U_1}{T_1}}{x_f}{C^\prime\,\tForall{x}{U_2}{T_2}}}

% \infrule[TFun$_{\textrm{id}}$]
% {
%   \subDft{S_2}{S_1} \\
%   \adpTyp{(\G, X <: S_2, z: T_1)}{z}{z}{T_2} \\
%   \subDft{C}{C^\prime}
% }
% {\adpDft{x}{C\,\tTForall{X}{S_1}{T_1}}{x}{C^\prime\,\tTForall{X}{S_2}{T_2}}}

\end{multicols}

\infrule[Fun]
{\adptDft{U_2}{U_1}{\cCat_1}{C_{e1}} \\
  \adpt{\G, x: U_2}{T_1}{T_2}{\cCat_2}{C_{e2}}\\
  % \sub{C \cup C_{e1} \cup C_{e2}}{C^\prime} \\
  \subDft{C \cup C_{e1} \cup C_{e2} / \set{x}}{C^\prime} \\
  \cCat^\prime = \begin{cases}
    \cVar, &\text{if both $\cCat_1$ and $\cCat_2$ are $\cVar$} \\
    \cVal, &\text{otherwise} \\
  \end{cases}
}
{\adptDft{C\,\tForall{x}{U_1}{T_1}}{C^\prime\,\tForall{x}{U_2}{T_2}}{\cCat^\prime}{C_{e1} \cup C_{e2}/\set{x}}}

\infrule[TFun]
{
  \subDft{S_2}{S_1} \\
  \adpt{\G, X <: S_2}{T_1}{T_2}{\cCat}{C_e} \\
  \subDft{C \cup C_e}{C^\prime} \\
  \cCat^\prime = \begin{cases}
    \cVar, &\text{if $\cCat$ is $\cVar$} \\
    \cVal, &\text{otherwise} \\
  \end{cases}
}
{\adptDft{C\,\tTForall{X}{S_1}{T_1}}{C^\prime\,\tTForall{X}{S_2}{T_2}}{\cCat^\prime}{C_e}}


\begin{multicols}{2}

\infrule[Box]
  {\adptDft{\tCap{C_1}{S_1}}{\tCap{C_2}{S_2}}{\cCat}{C_e} \\
  {C^\prime} \subseteq \dom{\G} \\
  % (\cCat^\prime, C_e^\prime) = \begin{cases}
  %   (\cVal, \eset), &\text{if $\cCat$ is $\cVar$} \\
  %   (\cTrm, \eset), &\text{if $\cCat$ is $\cVal$} \\
  %   (\cTrm, C_e), &\text{if $\cCat$ is $\cTrm$} \\
  % \end{cases}
  (\cCat^\prime, C_e^\prime) = \begin{cases}
    (\tBox{\cTrm}, \eset), &\text{if $\cCat \in \set{\cVar, \cVal}$} \\
    (\cCat, C_e),   &\text{otherwise}
  \end{cases}
  }
  {\adptDft{\tCap{C}{S}}{\tCap{C^{x}}{\tBox{\tCap{C^\prime}{S^\prime}}}}{\cCat^\prime}{{C_e^\prime}}}

\infrule[Unbox]
{
  \adptDft{\tCap {C_1} {S_1}}{\tCap{C_2}{S_2}}{\cCat}{C_e} \andalso
  {C_1} \subseteq \dom{\G}
}
{\adptDft{C_x\,\tBox{\tCap{C_1}{C_2}}}{\tCap{C_2}{S_2}}{\cTrm}{C_1 \cup C_e}}

\end{multicols}

\caption{Type-Level Box Adaptation System}
  \label{fig:adpt-sub}

\end{wide-rules}


==> figures/alt-typing.tex <==
\begin{wide-rules}

\textbf{Typing \quad $\typDft{t}{T}$}

\begin{multicols}{2}

\infrule[Var]
{\G(x) = \tCap CS}
{\typDft{x}{\tCapSet{x}{S}}}

  \infrule[Sub]
  {\typDft{t}{T} \\
  \subDft{T}{U}}
  {\typDft{t}{U}}

\infrule[Abs]
{\typ{\extendG{x}{U}}{t}{T} \\ \wfTyp{\G}{U}}
{\typDft{\tLambda{x}{U}{t}}{\tCap{\exclude{\cv{t}}{x}}{\tForall{x}{U}{T}}}}

\infrule[TAbs]
{\typ{\extendGT{X}{S}}{t}{T} \\ \wfTyp{\G}{S}}
{\typDft{\tTLambda{X}{S}{t}}{\tCap{\cv{t}}{\tTForall{X}{S}{T}}}}

\infrule[App]
{\typDft{x}{\tCap{C}{\tForall{z}{T}{U}}} \\
  \typDft{y}{T}}
{\typDft{x\ y}{\tSubst{z}{y}{U}}}

\infrule[TApp]
{\typDft{x}{\tCap{C}{\tTForall{X}{S}{T}}}}
{\typDft{x[S]}{\tSubst{X}{S}{U}}}

\infrule[Box]
{\typDft{x}{\tCap C S} \\ C \subseteq \dom{\G}}
{\typDft{\tBox{x}}{\tBox{\tCap C S}}}

\infrule[Unbox]
{\typDft{x}{\new{C_x}\,\tBox{\tCap C S}} \\ C \subseteq \dom{\G}}
{\typDft{\tUnbox{C}{x}}{\tCap{C}{S}}}

\end{multicols}

\infrule[Let]
{\typDft{s}{T} \\ \typ{\extendG{x}{T}}{t}{U}\\
  x \notin \fv{U}}
{\typDft{\tLet{x}{s}{t}}{U}}

\newruletrue
\infrule[Let$_{!}$]
{\typDft{y}{T} \\
 \typ{\extendG{x}{T}}{t}{U} \\}
{\typDft{\tLet{x}{y}{t}}{[x:=y]U}}
\newrulefalse

\caption{Type System (\system{})}
  \label{fig:alt-typing}

\end{wide-rules}


==> figures/cv.tex <==
\newcommand{\bbox}[1]{\mbox{\textbf{\textsf{#1}}}}
\newcommand{\OR}{\mathop{\ \ \ |\ \ \ }}

\begin{figure}[t]
  %\judgement{\textsf{Syntax}}{}
  %\vspace{-0.3em}
  \vspace{0.3em}
  \begin{center}\rule{1.0\textwidth}{0.4pt}\end{center}
  \vspace{0.3em}

  $\begin{array}[t]{llll@{\hspace{8mm}}l}
    \bbox{Variable} & \multicolumn{2}{l}{x, y, z} \\
    \bbox{Type Variable} & \multicolumn{2}{l}{X, Y, Z} \\[1em]
    \bbox{Value} & v, w & ::= & \lambda(x : T)t
        \OR \lambda[X \sub S]t
        \OR \new{\tBox{x}} \\

    \bbox{Answer} & a & ::= & v \OR x \\

    \bbox{Term} &s, t& ::= & a
          \OR  x\,y
          \OR  x\,[S]
          \OR  \tLet x s t
          \OR  \new{\tUnbox{C}{x}}\\

    \bbox{Shape Type} & S & ::= & X
          \OR  \top
          \OR  \forall(x : U) T
          \OR  \forall[X <: S] T
          \OR  \new{\tBox{T}} \\

    \bbox{Type} & T, U & ::= & S \OR \new{\tCap{C}{S}} \\

    \bbox{Capture Set} & \new{C} & ::= & \new{\{x_1, \ldots, x_n\}}
    \end{array}$

\caption{\label{fig:syntax} Syntax of \system{} and the box inference systems \cite{Odersky2022ScopedCF}}
\vspace{0.3em}
\begin{center}\rule{1.0\textwidth}{0.4pt}\end{center}
\vspace{0.3em}
\end{figure}

==> figures/subcapt.tex <==
\begin{wide-rules}

\textbf{Subcapturing \quad $\subDft{C_1}{C_2}$}

\begin{multicols}{2}

\infrule[Var]
{\G(x) = \tCap CS}
{\typDft{x}{\tCapSet{x}{S}}}

  \infrule[Sub]
  {\typDft{t}{T} \\
  \subDft{T}{U}}
  {\typDft{t}{U}}

\infrule[Abs]
{\typ{\extendG{x}{U}}{t}{T} \\ \wfTyp{\G}{U}}
{\typDft{\tLambda{x}{U}{t}}{\tCap{\exclude{\cv{t}}{x}}{\tForall{x}{U}{T}}}}

\infrule[TAbs]
{\typ{\extendGT{X}{S}}{t}{T} \\ \wfTyp{\G}{S}}
{\typDft{\tTLambda{X}{S}{t}}{\tCap{\cv{t}}{\tTForall{X}{S}{T}}}}

\infrule[App]
{\typDft{x}{\tCap{C}{\tForall{z}{T}{U}}} \\
  \typDft{y}{T}}
{\typDft{x\ y}{\tSubst{z}{y}{U}}}

\infrule[TApp]
{\typDft{x}{\tCap{C}{\tTForall{X}{S}{T}}}}
{\typDft{x[S]}{\tSubst{X}{S}{U}}}

\infrule[Box]
{\typDft{x}{\tCap C S} \\ C \subseteq \dom{\G}}
{\typDft{\tBox{x}}{\tBox{\tCap C S}}}

\infrule[Unbox]
{\typDft{x}{\new{C_x}\,\tBox{\tCap C S}} \\ C \subseteq \dom{\G}}
{\typDft{\tUnbox{C}{x}}{\tCap{C}{S}}}

\end{multicols}

\infrule[Let]
{\typDft{s}{T} \\ \typ{\extendG{x}{T}}{t}{U}\\
  x \notin \fv{U}}
{\typDft{\tLet{x}{s}{t}}{U}}

\newruletrue
\infrule[Let$_{!}$]
{\typDft{y}{T} \\
 \typ{\extendG{x}{T}}{t}{U} \\}
{\typDft{\tLet{x}{y}{t}}{[x:=y]U}}
\newrulefalse

\caption{Type System (\system{})}
  \label{fig:alt-typing}

\end{wide-rules}


==> sections/capset-inference.tex <==
\section{Capture Set Inference}



==> sections/cc-adp.tex <==
\subsection{\ccAdp{}: Box Inference for \ccAlgo{}}

\input{sections/cc-adp/presentation.tex}

\input{sections/cc-adp/metatheory.tex}



==> sections/cc-adp/presentation.tex <==
% \subsection{Formal Presentation}

% \input{figures/adp-typ.tex}

% \input{figures/adp-sub.tex}

Figure \ref{fig:adp-typ} presents the type system \ccAdp{} with box inference.
Figure \ref{fig:adp-sub} presents the box adaptation system.

% \subsubsection{Avoidance with simplification}

% \begin{equation*}
% 	\substLocal{t}{T} =
%   \begin{cases}
%     ([x:=y]u, [x:=y]U), &\text{if $t$ is of form $\tLet{x}{y}{s}$ and $(u, U) = \substLocal{s}{T}$}, \\
%     (\tLet{x}{u}{s^\prime}, U), &\text{if $t$ is of form $\tLet{x}{s}{s^\prime}$ and $(u, U) = \substLocal{s^\prime}{T}$}, \\
%     (t, T), &\text{otherwise}.
%   \end{cases}
% \end{equation*}

% \begin{equation*}
% 	\avoidPrec{x}{U}{t}{T} =
%   (t^\prime, \avoidOp{x}{U}{T^\prime}),
%   % \begin{cases}
%   %   ([x := y]s, [x := y]T), &\text{if $t$ is of form $\tLet{x}{y}{s}$},\\
%   %   abc, &\text{if $t$ is of form $\tLet{y}{s}{u}$ and $(u^\prime, T^\prime)$}.\\
%   % \end{cases}
% \end{equation*}
% where $(t^\prime, T^\prime) = \substLocal{t}{T}$.

% \begin{equation*}
% \simpLet{\G}tT =
% \begin{cases}
% ([x:=y]u, [x:=y]U), &\text{if $t$ is of form $\tLet{x}{y}{s}$ and $(u, U) = \simpLet{\G}sT$},\\
% (\tLet{x}{s}{u}, \avoidOp{\G}{x}{U}), &\text{if $t$ is of form $\tLet{x}{s}{s^\prime}$ and $(u, U) = \simpLet{\G}{s^\prime}{T}$}),\\
% (t, T), &\text{otherwise}.\\
% \end{cases}
% \end{equation*}

\subsubsection{Compacting adapted terms}

\begin{equation*}
  \compact{t} =
  \begin{cases}
  \compactLet{\tLet{x}{\compact{s}}{\compact{t}}}, &\text{if $t$ is of form $\tLet{x}{s}{t}$}, \\
  \compactLam{\tLambda{z}{T}{(\compact{s})}}, &\text{if $t$ is of form $\tLambda{z}{T}{s}$},\\
  t,  &\text{otherwise}.\\
  \end{cases}
\end{equation*}

\begin{equation*}
  \compactLet{t} =
  \begin{cases}
    x, &\text{if $t$ is of form $\tLet{y}{\tUnbox{C}{x}}{\tBox{y}}$}, \\
    t, &\text{if $t$ is of form $\tLet{y}{t}{y}$},\\
    [x := y] t, &\text{if $t$ is of form $\tLet{x}{y}{t}$},\\
    t,  &\text{otherwise}.\\
  \end{cases}
\end{equation*}

\begin{equation*}
  \compactLam{t} =
  \begin{cases}
    x, &\text{if $t$ is of form $\tLambda{z}{T}{x\,z}$}, \\
    x, &\text{If $t$ is of form $\tTLambda{X}{S}{x[X]}$}, \\
    t,  &\text{otherwise}.\\
  \end{cases}
\end{equation*}




==> sections/cc-algo.tex <==
\subsection{\ccAlgo{}: Semi-Algorithmic Typing for \cc{}}

% \input{sections/cc-algo/presentation.tex}

\input{sections/cc-algo/proof.tex}



==> sections/cc-algo/presentation.tex <==
% \subsection{Formal Presentation}

% \input{figures/algo-typing.tex}

% \input{figures/var-typing.tex}

% The semi-algorithmic type system is presented in Figure \ref{fig:algo-typing}.
% The rules for type variables are presented in Figure \ref{fig:var-typing}.



==> sections/cc-alt.tex <==
\subsection{An Alternative Variant of \system{}}

\input{figures/alt-typing.tex}




==> sections/formal-v1.tex <==
\section{Formal Presentation}

% \input{sections/cc-alt.tex}

\input{sections/cc-algo.tex}

\input{sections/cc-adp.tex}

\input{sections/cc-adpt.tex}



==> sections/informal-v1.tex <==
\section{Informal Introduction to \ccAdp{}}

\ccAdp{} is a system that formalises box inference in \cc{}.
It extends \cc{} with the ability to infer box and unbox expressions to transform a term to be well-typed in \cc{}.
Also, it makes the typing rules syntax-direct so that it directly gives rise to a semi-algorithm for box inference.
In this section, we informally introduce the \ccAdp{} system.
We start with a explanation of what box inference is and why we need it.
Then, we explain the main concepts and features of the box inference system.
We finally introduce the type-level variant of \ccAdp{},
which mimics the effect of box inference on the type level only without actually modifying the terms.

\subsection{Problem Formulation}

% Why box inference?
Capture calculus has box constructs on both the type and the term level (i.e. boxing-, unboxing- expressions and boxed types).
However, in the implementation, to reduce users' notational burden,
we hope that the box constructs do not have to be written out explicitly.
Scala 3, which has a full implementation of capture checking, completely omits the notion of boxes in its syntax, and does box inference to complete all the box constructs for the users.
Specifically, given a user-written program in a surface language without box constructs, box inference aims to figure out a semantic-preserving program with box constructs properly inserted, being a valid program in the core calculus \cc{}.
In the following we inspect a concrete example of box inference, which is written in pseudo-Scala syntax and encodes tuples in church encoding.
\begin{minted}{scala}
type Top = {*} Any

type Tuple[A <: Top, B <: Top] = [C] -> (A => B => C) -> C
def makeTuple[A <: Top, B <: Top](a: A, b: B): Tuple[A, B] =
  [C] => f => f(a)(b)

def main(io: {*} Cap, logger: {io} Logger) = {
  val t1 = makeTuple[{io} Cap, {io} Logger](io, logger)
}
\end{minted}

In order to make it well-typed in \cc{}, the program will be transformed into the following one with box inference:
\begin{minted}[escapeinside=||]{scala}
type Top = {*} Any

type Tuple[A <: |$\new{\Hsquare}$| Top, B <: |$\new{\Hsquare}$| Top] = [C] -> (A => B => C) -> C
def makeTuple[A <: |$\new{\Hsquare}$| Top, B <: |$\new{\Hsquare}$| Top](a: A, b: B): Tuple[A, B] =
  [C] => f => f(a)(b)

def main(io: {*} Cap, logger: {io} Logger) = {
  val t1 = makeTuple[|$\new{\Hsquare}$| {io} Cap, |$\new{\Hsquare}$| {io} Logger](|$\new{\Hsquare}$| io, |$\new{\Hsquare}$| logger)
}
\end{minted}
Note the box constructs we inserted for the program, which is highlighted in grey.
In \ccAdp{}, we focus on the formalisation of how we infer the box constructs on terms, i.e. the last two boxes in the above example.
Now, we are ready to define the problem that box inference aims to solve.

\emph{Problem of box inference.}
Given a program with with missing box constructs, and possibly ill-typed, we would like to output a program by inserting box, unbox, and eta-expansion on the input program to make it well-typed in capture calculus.

Note that we use eta-expansions for box inference over functions.
We can see this in the following example, which is extended from the example we give above:
\begin{minted}{scala}
  /* ... */

  def main(io: {*} Cap, logger: {io} Logger) = {
    val t1 = makeTuple[{io} Cap, {io} Logger](io, logger)

    def useLogger(_: {io} Cap)(l: {io} Logger): Unit = l.log(0)

    t1[Unit](useLogger)
  }
\end{minted}

In the line where we call the tuple with \scalacode{useLogger}, the expected type of \scalacode{useLogger} here is \mintinline[escapeinside=||]{scala}{(|$\Hsquare$| {io} Cap) => (|$\Hsquare$| {io} Logger) => Unit}.
However, the actual type of \scalacode{useLogger} is \scalacode{({*} Cap) => ({io} Logger) => Unit}.
It turns out that it is only possible to adapt the \scalacode{useLogger} into its expected term by eta-expansion.
Specifically, \scalacode{t1[Unit](useLogger)} should be transformed to the following term:
\begin{minted}[escapeinside=||]{scala}
t1[Unit](x => y => useLogger(|$\tUnbox{\set{io}}{}$| x)(|$\tUnbox{\set{io}}{}$| y))
\end{minted}
In the transformed term, we eta-expand \scalacode{useLogger} and insert unbox operations on the arguments to make the function conform to the expected type.

\subsection{Main Concepts}

\ccAdp{} is an extension of the type system of \cc{}.
Its typing rules are based on those of \cc{}, but it has the capability of inferring box constructs on terms.
Now, we informally discuss the main concepts of \ccAdp{}.

\textbf{Term transformation during typing.}
\ccAdp{} fuses typing and box inference.
When typing a term, \ccAdp{} not only derives a type for it, but also transforms it by inserting box-related constructs.
Specifically, given a term $t$, \ccAdp{} tries to derive a type $T$ for it and at the same time transform it into $t^\prime$.
A well-typed $t$ in \ccAdp{} may be ill-typed in \cc{} due to missed box constructs, but the transformed term $t^\prime$ always conforms to the derived type $T$ in the \cc{} system.

\textbf{Subtyping with box adaptation.}
In \ccAdp{}, the insertion of box-related constructs happens when we are typing an application, when we have an expected type for the argument.
For example, in the previous example, when we are typing the function application:
\begin{minted}[escapeinside=||]{scala}
t1[Unit](useLogger)
\end{minted}
we have to check whether the actual type of the variable \scalacode{useLogger} conforms to the expected type, which comes from the type signature of the function.
In \cc{} we use subtyping for this.
Mismatched boxes leads to type errors.
In \ccAdp{}, we extend subtyping with the ability of doing box adaptation, i.e. inserting box-related constructs on the term.
Given a variable $x$ with its actual type $T$ and the expected type $U$, \ccAdp{} subtyping checks whether the variable can be adapted to the expected type with regular subtyping reasoning along with box adaptation transformations, and returns the transformed term $t^\prime$ built from $x$.
$t^\prime$ has all the mismatches between boxes fixed and is well-typed as the expected type $U$ in \cc{} system.
We name this extended variant of subtyping \emph{box adaptation}.
Back to the example, when checking \scalacode{useLogger} against the expected type with box adaptation, we adapt it into \mintinline[escapeinside=||]{scala}{x => y => useLogger(|$\tUnbox{\set{*}}{}$| x)(|$\tUnbox{\set{io}}{}$| y)}.
When talking about box adaptation, we always assume that the term to be adapted is a variable.
This simplifies the presentation without the loss of generality, as we can always lcaolly bind a term to a variable, and it aligns well with the ANF formulation of \cc{}.

\textbf{Box adaptation.}
Now we lay out the basic idea of box adaptation.
The basic case is when the actual and expected type differs in term of whether they are boxed.
In the first example, in the application \mintinline{scala}{makeTuple[...](io, logger)}, the expected type of \scalacode{io} is \tBox{\mintinline{scala}{{*} Cap}}, while the actual type is just \mintinline{scala}{{io} Cap}.
Box adaptation infers a box here.
Functions are non-trivial to be box-adapted.
As explained before, we have to eta-expand functions when box-adapting them.
Notably, box inference fails when it is necessary to box or unbox a variable that captures the universal capability.
For example, it is impossible to adapt a variable of \mintinline{scala}{({*} Cap) => Unit} into \mintinline[escapeinside=||]{scala}{(|$\tBox{}$| {*} Cap) => Unit},
since unboxing the argument of the eta-expanded function (i.e. \mintinline[escapeinside=||]{scala}{(x: |$\Hsquare$| {*} Cap) => f(|$\tUnbox{\set{*}}{}$| x)}), which captures the universal capability, is disallowed in capture calculus.

\subsection{Type-Level Box Inference}

Box constructs do not change the runtime behavior of programs.
In other words, the transformation on programs we perform during box inference does not impact semantics.
In fact, the implementation of capture checking in Scala does not have boxes on terms, and only use a boolean value to indicate whether a type is boxed.
For time and space efficiency, it would be natural to ask whether it is possible to perform box inference on the type level only, without actually transforming the terms?

The answer is yes. In this section, we informally introduce \ccAdpt{}, which is a variant of \ccAdp{} that formalizes the inference of boxes equivalent to what \ccAdp{} does, but only on the type level.
Specifically, it also has the adaptation subtyping and typing rules as \ccAdp{} does, but the adaptation rules checks whether a type can be box-adapted to the expectation without reasoning about and transforming the actual term.
\ccAdpt{} achieves this by simulating the effects of boxes on the type level without really transforming the terms.

\subsubsection{Type-Level Effects of Box Adaptation}
We start by discussing the ways term-level box adaptation can impact the types.
Box adaptation preserves the general structures of the terms' types (i.e. that functions can still be typed as functions after box adaptation).
The only effect we need to pay attention to is that box adaptation changes the captured variables of a term.
To see an example, when adapting a variable \scalacode{f} of type \scalacode{(x: {io} Logger) -> Unit} into the expected type \mintinline[escapeinside=||]{scala}{{io} (x: |$\tBox{}$| {io} Logger) -> Unit}, the result of term-level box adaptation will be:
\begin{minted}[escapeinside=||]{scala}
(x: |$\tBox{}$| {io} Logger) => f(|$\tUnbox{\set{io}}{x}$|)
\end{minted}
Its captured variables are $\set{io, f}$.
It \emph{additionally} captures \texttt{io} compared to the original one.
The change of term's captured variable affects types in two ways:
\begin{itemize}
  \item The capture set in the type of the adapted term changes, thus posing additional constraints on the capture set of the expected type. The previous example already illustrates this: the capture set of the expected function type must include \texttt{io} because of the box adaptation while the orginal function is pure.

  \item Adapted terms may be part of the body of a function, thus changing the capture set of that function.
    To see a concrete example, consider the following code:
    \begin{minted}{scala}
/* ... */

def main(io: {*} Cap, logger: {io} Logger) = {
  val t1 = makeTuple[{io} Cap, {io} Logger](io, logger)

  def useLogger(_: {io} Cap)(l: {io} Logger): Unit = l.log(0)

  (x: Unit) => t1[Unit](useLogger)
}
    \end{minted}
    When typing the body of the function \scalacode{(x: Unit) => t1[Unit](useLogger)}, \scalacode{useLogger} is adapted into 
\begin{minted}[escapeinside=||]{scala}
x => y => useLogger(|$\tUnbox{\set{io}}{}$| x)(|$\tUnbox{\set{io}}{}$| y)
\end{minted}
    and thus additionally captures \texttt{io}.
    In the end, the type of the function will be \scalacode{{io} Unit -> Unit}.
\end{itemize}

% Term-level box adaptation does not change the general structure of the type of the term execpt for the boxes.
% For example, terms of function types continue to be functions after box adaptation with the boxes inserted into or removed from types.
% The most essential impact box adaptation have on types is the change of \emph{capture sets} in them.
% This is because inserting an unbox in term will result in a term with a more variables captured; also, inserting a box can reduce the captured variable set.
% The changes in the captured variable set impact the capture set of their types.
% For example, when adapting a variable \scalacode{f} of type \scalacode{(x: {io} Logger) -> Unit} into the expected type \mintinline[escapeinside=||]{scala}{{io} (x: |$\tBox{}$| {io} Logger) -> Unit}, the result of term-level box adaptation will be:
% \begin{minted}[escapeinside=||]{scala}
% (x: |$\tBox{}$| {io} Logger) => f(|$\tUnbox{\set{io}}{x}$|)
% \end{minted}
% Note that the insertion of the unbox operation makes the result term to additionally capture the set $\set{io}$.
% As a result, the expected function type captures $\set{io}$ despite that the unadapted function is pure, otherwise it would fail the type checking.
% Type-level box inference have to keep track of these effects on capture set.
% Now we discuss these effects in details.
Next, we discuss the effects box adaptation have on capture sets.

\paragraph{Top-level boxes}
We observe that the set of captured variables is always enlarged by box adaptation unless a box is inserted at the top-level.
Specifically, given a variable $x$, the term $t$ obtained from box-adapting $x$ always captures $x$ itself, unless $x$ is adapted to $\tBox{x}$.
We name the case where $x$ is adapted to $\tBox{x}$ \emph{top-level boxes}.
In other words, we always charge the capture set in the type and the environment with more variables unless it has a top-level box inserted.

\paragraph{Capture leackage from unboxing}
Inserting an unbox enlarges the set of captured variables.
This results in a larger capture set in types and charges more variables to the closure.
The previous example demonstrates such effects.
Specifically, if we infer an unbox for a variable of type $\tUnbox{C}{S}$, the adapted term additionally captures $C$ and charge capture sets of types and closures.
% Specifically, infer an unbox operation on a term leaks the boxed capturing set to the types which the adapted term is part of.
Take the adaptation of functions as an example.
Generally, if we are adapting a function of actual type \scalacode{C1 T1 -> U1} to the expected type \scalacode{C2 T2 -> U2}, the type of the result should capture the additional captured variables resulted from the adaptation of \scalacode{T1} and \scalacode{U1}, and the outer closure would capture these variables too.
We call the effects from unboxing \emph{capture leackage}, in that unbox operations \emph{leaks} the boxed capture set to types and the outer closure.

\paragraph{Boxes stop capture leakage}
Inferring a box on a term blocks the captured variables leaked during the adaptation of that term from escaping to the capture set of outer types and closures.
To see a concrete example, when adapting a function \scalacode{f} of the type \scalacode{Unit -> (x: {io} Logger) -> Unit}, a possible expected type can be \mintinline[escapeinside=||]{scala}{{io} Unit -> {io} (x: |$\tBox{}$| {io} Logger) -> Unit}.
The result of term-level adaptation would be \mintinline[escapeinside=||]{scala}{(_: Unit) => (x: |$\tBox{}$| {io} Logger) => f(|$\tUnbox{\set{io}}{}$| x)}.
Note how the expected types captures $\set{io}$ additionally in two different places.
However, another possible expected type can be \mintinline[escapeinside=||]{scala}{{} Unit -> |$\tBox{}$| {io} (x: |$\tBox{}$| {io} Logger) -> Unit}.
The adapted term, in this case, is \mintinline[escapeinside=||]{scala}{(_: Unit) => |$\tBox{}$| (x: |$\tBox{}$| {io} Logger) => f(|$\tUnbox{\set{io}}{}$| x)}.
The box we inferred here stops the leaked capture set $\set{io}$ from charging the outermost capture set.

\subsubsection{Main Ideas of Type-Level Box Adaptation and Box Inference}

The ideas of top-level boxes and capture leakage leads us to the type-level system for box inference.
Now we discuss the main ideas of it.

\paragraph{Tracking capture leakage in box adaptation}
Based on the observation we had before, we only need to track the leaked variable in the rules and require the capture set of the expected type to include the leaked captured variables in type-level box adaptation.
We enlarge the leaked variable set when an unbox construct is inferred and clear the leaked set when a box is inserted.
This will suffice to mimic term-level adaptation.

\paragraph{Typing with Type-Level Box Inference}
Typing rules in \ccAdp{} returns an box-adapted term that conforms to the derived type.
Differently, in the type-level system, the typing rules keep track of the captured variable of the adapted term without actually constructing it.
When invoking the adaptation subtyping rule when typing function applications, we compute the captured variable of the adapted term from the set of leaked variables derived by type-level box adaptation.

In the following section, we will formally prove the equivalence between the type-level system and the term-level one.
Notably, the design of the type-level box adaptation aligns surprisingly well with the Scala implementation of capture checking and box inference.

% 1. Box adaptation does not change the general structure of types, except for boxes.
% 2. The key effects are on the captured variables of terms and capture sets of types.
% 3. How do box adaptation change capture sets?
% 4. Unboxing a term makes it captures more variables.
% 5. Boxing a term stops it from capturing more.
% 6. The type-level system mimics the effect of term-level box adaptation by tracking the additional captured variables induced by boxing and unboxing.


